How Does Naming Affect LLMs on Code Analysis Tasks?

The Large Language Models (LLMs), such as GPT and BERT, were proposed for natural language processing (NLP) and have shown promising results as general-purpose language models. An increasing number of industry professionals and researchers are adopting LLMs for program analysis tasks. However, one significant difference between programming languages and natural languages is that a programmer has the flexibility to assign any names to variables, methods, and functions in the program, whereas a natural language writer does not. Intuitively, the quality of naming in a program affects the performance of LLMs in program analysis tasks. This paper investigates how naming affects LLMs on code analysis tasks. Specifically, we create a set of datasets with code containing nonsense or misleading names for variables, methods, and functions, respectively. We then use well-trained models (CodeBERT) to perform code analysis tasks on these datasets. The experimental results show that naming has a significant impact on the performance of code analysis tasks based on LLMs, indicating that code representation learning based on LLMs heavily relies on well-defined names in code. Additionally, we conduct a case study on some special code analysis tasks using GPT, providing further insights.

==> Makefile <==
PAPER = main
REFERENCE = main
JUNK =*.log *.synctex\(busy\) *.xml *.bcf *.toc *.snm *.nav *.fls *.fdb_latexmk *.synctex.gz *.spl *.ps *.dvi  *.out *.aux *.backup *~ *.blg
COUNTING_TOOL = ./texcount.pl
TEMP = 0
MY_VAR=$(shell echo whatever)

# Define the tools we are going to use

all: pdf

# Rules for various parts of the target
pdf: $(PAPER).tex
	pdflatex $(PAPER).tex
	bibtex $(PAPER).aux
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex
	#rm -f $(JUNK)

clean:
	rm -f $(JUNK) $(PAPER).pdf




==> backround.tex <==
\section{Background}
\subsection{Large Language Model and Program Analysis}
Large language models has been widely used to generate, analyze programs. 
CodeBert purposed by XXX leverage the Bert that trained on a 
 and GraphCodeBert p
\subsection{ChatGPT for Coding}

``In its current state, we believe that GPT-4 has a high proficiency in writing focused programs that only depend on existing public libraries, which favorably compares to the average software engineer’s ability."~\cite{bubeck2023sparks}.
``We also acknowledge that GPT-4 is not perfect in coding yet, as it sometimes produces syntactically invalid or semantically incorrect code, especially for longer or more complex programs.''

``GPT-4 also sometimes fails to understand or follow the instructions, or produces code that does not match the in- tended functionality or style. With this acknowledgment, we also point out that GPT-4 is able to improve its code by responding to both human feedback (e.g., by iteratively refining a plot in 3.2) and compiler / terminal errors (examples in Section 5.1)."
\subsection{ChatGPT for Code Analysis}

==> sections/case-fuzzing.tex <==
\vspace{-0.5em}\subsection{Input Generation}
Input generation is wide used in software testing, which aim to achieve a high coverage by triggering different program pathes.
This section, we aim to answer \ding{188} whether ChatGPT can offer valuable and effective seed inputs after understanding the source code.
Specifically, we test the ChatGPT's input generatation ability to achieve code coverage, input mutations, and  exeuction simulation.

Upon analyzing the responses ({\bf \ref{appendix:Q11}, \ref{appendix:Q12}, \ref{appendix:Q13}}) from ChatGPT, we observed that the provided seeds were comparable to those generated by AFL (American Fuzzy Lop) \cite{aflrefurl} using seed mutation strategies. However, it became apparent that ChatGPT did not propose highly effective seeds (capable of triggering the vulnerability). This observation suggests that ChatGPT may face challenges in leveraging the program semantics it learned from the code to generate such effective seeds.
There could be two possible reasons for this:

\begin{enumerate}
\item The prompts we use may not have been designed to specifically encourage ChatGPT to produce the most useful and targeted solutions.\lan{remove this. if it is true, we could say our previous case studies are not correct because of prompts. this is out-of-scope}
\item ChatGPT's responses might be too general, primarily relying on the information present in the corpus it was trained on, rather than effectively applying the learned program semantics to new situations.
\end{enumerate}

\lan{I vote to remove this. then we only have to kinds of case study: semantic and vunlerbiltiy. it would be easier to explain the storyline}
%Understanding these limitations is crucial for utilizing ChatGPT effectively in vulnerability discovery and other security-oriented tasks. Further research is needed to refine the prompts and explore strategies to enhance ChatGPT's ability to provide more precise and context-aware responses in security-related scenarios.



==> sections/preliminary.tex <==
% \section{Terminologies}
\vspace{-0.5em}
\section{Literal Features and Logic Features}

% A source code file in a program consists of a sequence of strings, which can be grouped into three categories: keyword, operator, (both are defined in the programming language specification) and developer-defined name.
% Keywords are reserved words that have special meanings and can only be used for specific purposes.
% For example, \texttt{for}, \texttt{if}, and \texttt{break} are widely known keywords in many programming languages.
% They are used in a program to change the control flow.
% The number of keywords is limited in a programming language.
% For instance, \texttt{C} programming language has 32 keywords and \texttt{Python} (version 3.7) has 35 keywords.
% Besides keywords, a programming language needs to define a set of operators, representing operations and actions.
% For example, arithmetic operators (\eg, \texttt{+}, \texttt{-}, and \texttt{*}) and logical operators (\eg, \texttt{and}, \texttt{or}, and \texttt{not}) are two of most important categories.
% In addition, a developer can use any string to name a variable, structure, function, class, etc., as long as this string is not conflicted with reserved keywords and operators, and follows the programming language specification.

% When writing code, due to the program logic, the developer has limited flexibility to choose keywords and operators.
% Only some keywords (such as \texttt{for} and \texttt{while}) and operators (such as \texttt{++}, \texttt{+1}) are exchangeable.
% That is, the program logic is fixed when using a set of keywords and operators in a program.
% In contrast, the name of a variable, function, or class has no impact on the program logic.

% \lstset{style=mycstyle}
% \begin{lstlisting}[language=C++,
% emph={bubble_sort, begin, end, pred, it_end, finished, next, it},
% label={code:goodname},caption={A piece of code with meaningful variable/function names.}, captionpos=b]{}
%     void bubble_sort(It begin, It end, Pred pred=Pred()){
%         if ( std::distance( begin, end ) <= 1 ){ return; }
%         auto it_end    = end;
%         bool finished  = false;
%         while ( !finished ){ //loop stop when no adjacent elements are not in required order. 
%             ...
%         }   
%     }
% \end{lstlisting}


% \begin{lstlisting}[language=C++,
% emph={var1, var2, var3, var4, var5, var6, fun1, fun2},
% label={code:badname},caption={The same code without meaningful variable/function names.}, captionpos=b]{}
%     void fun1(It var1, It var2, Pred fun2=Fun2()){
%         if ( std::distance( var1, var2 ) <= 1 ){ return; }
%         auto var3  = var2;
%         bool var4  = false;
%         while ( !var4 ){
%             ...
%         }   
%     }
% \end{lstlisting}

% % \textcolor{red}{(Where is this bubble sorting function from? C++ standard library? Can we add some comments, i.e., programmer-readable annotation?)}
% \autoref{code:goodname} and \autoref{code:badname} are two pieces of code with the same program logic~\textendash~\textit{bubble sorting}.
% \autoref{code:goodname} is an implementation from the Web, which has well-named functions and variables whereas \autoref{code:badname} is anonymized by us. 
% Through a quick glance, even a novice can easily conclude that \autoref{code:goodname} is a bubble-sort function based on the help from the literal meaning of the function name and the variable names.
% However, it needs more time for an experienced analyst to go through this function line by line to understand the purpose of \autoref{code:badname}. 
% Therefore, despite the exactly same program logic, \autoref{code:badname} is much more difficult to analyze.
% In summary, although the name of a variable, function, or class has no impact on the program logic, it could also help the analyst to understand the purpose of a program if the literal meaning of the name aligns with the program logic.

% From the above discussion, we give the definition of literal features and logical features:

\begin{definition}[Literal Features and Logical Features]
Given a piece of code, the \textbf{literal features} are features of the literal meaning of the variable names, function names and programmer-readable annotation. These feature could be removed without change the functionality of the code. The \textbf{logical features} are features that control the program logic. The keywords and operators defined by a programming language specification are logical features.
\end{definition}

%Based on this definition, we can draw the following conclusions from our experiments:%. Two kinds of code snippets are analyzed: 
Based on this definition, we have the following observations:
1) code snippets can be understood in two ways: \textit{literal analysis}, and \textit{logic analysis};  2) the literal analysis makes a conclusion based on the names of variables, functions, etc., which is easier to analyze but is not always reliable; 3) the logic analysis requires a high-level understanding of the code, which is more reliable but hard to analyze.



